Ideological Ambiguity and Political Spectrum

This study examines the relationship between ambiguity and the ideological positioning of political parties across the political spectrum. We identify a strong non-monotonic (inverted U-shaped) relationship between party ideology and ambiguity within a sample of 202 European political parties. This pattern is observed across all ideological dimensions covered in the data. To explain this pattern, we propose a novel theory that suggests centrist parties are perceived as less risky by voters compared to extremist parties, giving them an advantage in employing ambiguity to attract more voters at a lower cost. We support our explanation with additional evidence from electoral outcomes and economic indicators in the respective party countries.

==> table1Bapp.tex <==
Position on social values&       0.020         &       1.459\sym{***}&       1.264\sym{***}&       1.264\sym{***}&                     \\
                    &     (0.029)         &     (0.153)         &     (0.146)         &     (0.146)         &                     \\
Position on social values sq.&                     &      -0.138\sym{***}&      -0.121\sym{***}&      -0.121\sym{***}&                     \\
                    &                     &     (0.015)         &     (0.014)         &     (0.014)         &                     \\
Centrism on social values&                     &                     &                     &                     &       0.819\sym{***}\\
                    &                     &                     &                     &                     &     (0.088)         \\
Joint significance  &                     &       0.000         &       0.000         &       0.000         &                     \\
Vertex              &                     &       5.285         &       5.236         &       5.236         &                     \\
R-squared           &       0.527         &       0.473         &       0.652         &       0.652         &       0.688         \\
Observations        &         253         &         253         &         253         &         253         &         253         \\


==> table2Aa.tex <==
Position on economic issues&       0.043         &       1.617\sym{***}&       1.492\sym{***}&       1.492\sym{***}&                     \\
                    &     (0.042)         &     (0.174)         &     (0.207)         &     (0.207)         &                     \\
Position on economic issues sq.&                     &      -0.161\sym{***}&      -0.149\sym{***}&      -0.149\sym{***}&                     \\
                    &                     &     (0.018)         &     (0.021)         &     (0.021)         &                     \\
Centrism on economic issues&                     &                     &                     &                     &       0.594\sym{***}\\
                    &                     &                     &                     &                     &     (0.103)         \\
Joint significance  &                     &       0.000         &       0.000         &       0.000         &                     \\
Vertex              &                     &       5.014         &       4.995         &       4.995         &                     \\
R-squared           &       0.469         &       0.316         &       0.595         &       0.595         &       0.546         \\
Observations        &         259         &         259         &         259         &         259         &         259         \\


==> table2Bb.tex <==
Position on social values&       0.020         &       1.459\sym{***}&       1.264\sym{***}&       1.264\sym{***}&                     \\
                    &     (0.029)         &     (0.153)         &     (0.146)         &     (0.146)         &                     \\
Position on social values sq.&                     &      -0.138\sym{***}&      -0.121\sym{***}&      -0.121\sym{***}&                     \\
                    &                     &     (0.015)         &     (0.014)         &     (0.014)         &                     \\
Centrism on social values&                     &                     &                     &                     &       0.819\sym{***}\\
                    &                     &                     &                     &                     &     (0.088)         \\
Joint significance  &                     &       0.000         &       0.000         &       0.000         &                     \\
Vertex              &                     &       5.285         &       5.236         &       5.236         &                     \\
R-squared           &       0.527         &       0.473         &       0.652         &       0.652         &       0.688         \\
Observations        &         253         &         253         &         253         &         253         &         253         \\


==> table3A.tex <==
Position on economic issues&       0.028\sym{**} &       0.428\sym{***}&       0.378\sym{***}&       0.350\sym{***}&      -0.038         &       0.498\sym{***}\\
                    &     (0.011)         &     (0.044)         &     (0.042)         &     (0.041)         &     (0.042)         &     (0.087)         \\
Position on economic issues sq.&                     &      -0.043\sym{***}&      -0.037\sym{***}&      -0.034\sym{***}&                     &      -0.053\sym{***}\\
                    &                     &     (0.005)         &     (0.004)         &     (0.004)         &                     &     (0.008)         \\
Joint significance  &                     &       0.000         &       0.000         &       0.000         &                     &       0.000         \\
Vertex              &                     &       4.997         &       5.073         &       5.119         &                     &       4.679         \\
R-squared           &       0.330         &       0.160         &       0.336         &       0.413         &       0.764         &       0.788         \\
Observations        &        1101         &        1101         &        1101         &        1101         &         960         &         960         \\


==> table3B.tex <==
Position on social values&  -0.016\sym{\dagger}&       0.492\sym{***}&       0.464\sym{***}&       0.460\sym{***}&      -0.047         &       0.701\sym{***}\\
                    &     (0.010)         &     (0.033)         &     (0.037)         &     (0.034)         &     (0.039)         &     (0.085)         \\
Position on social values sq.&                     &      -0.048\sym{***}&      -0.046\sym{***}&      -0.046\sym{***}&                     &      -0.072\sym{***}\\
                    &                     &     (0.003)         &     (0.004)         &     (0.003)         &                     &     (0.008)         \\
Joint significance  &                     &       0.000         &       0.000         &       0.000         &                     &       0.000         \\
Vertex              &                     &       5.097         &       5.012         &       5.015         &                     &       4.875         \\
R-squared           &       0.279         &       0.256         &       0.374         &       0.476         &       0.713         &       0.779         \\
Observations        &        1102         &        1102         &        1102         &        1102         &         962         &         962         \\


==> table3C.tex <==
Position on multiculturalism&      -0.065\sym{***}&       0.474\sym{***}&       0.467\sym{***}&       0.420\sym{***}&      -0.092\sym{**} &       0.918\sym{***}\\
                    &     (0.014)         &     (0.049)         &     (0.054)         &     (0.037)         &     (0.044)         &     (0.118)         \\
Position on multiculturalism sq.&                     &      -0.048\sym{***}&      -0.048\sym{***}&      -0.043\sym{***}&                     &      -0.093\sym{***}\\
                    &                     &     (0.005)         &     (0.005)         &     (0.004)         &                     &     (0.012)         \\
Joint significance  &                     &       0.000         &       0.000         &       0.000         &                     &       0.000         \\
Vertex              &                     &       4.952         &       4.919         &       4.825         &                     &       4.943         \\
R-squared           &       0.398         &       0.194         &       0.361         &       0.506         &       0.678         &       0.756         \\
Observations        &        1087         &        1088         &        1088         &        1087         &         946         &         946         \\


==> table4A.tex <==
Position overall    &       0.008         &       0.232\sym{***}&       0.147\sym{***}&       0.119\sym{***}&      -0.000         &       0.577\sym{***}\\
                    &     (0.009)         &     (0.057)         &     (0.034)         &     (0.033)         &     (0.052)         &     (0.122)         \\
Position overall sq.&                     &      -0.021\sym{***}&      -0.014\sym{***}&      -0.011\sym{***}&                     &      -0.055\sym{***}\\
                    &                     &     (0.005)         &     (0.004)         &     (0.003)         &                     &     (0.011)         \\
Joint significance  &                     &       0.001         &       0.000         &       0.001         &                     &       0.000         \\
Vertex              &                     &       5.496         &       5.414         &       5.505         &                     &       5.220         \\
R-squared           &       0.310         &       0.049         &       0.225         &       0.321         &       0.794         &       0.814         \\
Observations        &        1101         &        1101         &        1101         &        1101         &         962         &         962         \\


==> table4B.tex <==
Position on immigration&      -0.038\sym{***}&       0.454\sym{***}&       0.414\sym{***}&       0.375\sym{***}&      -0.095\sym{**} &       0.784\sym{***}\\
                    &     (0.009)         &     (0.026)         &     (0.025)         &     (0.030)         &     (0.043)         &     (0.101)         \\
Position on immigration sq.&                     &      -0.044\sym{***}&      -0.041\sym{***}&      -0.037\sym{***}&                     &      -0.080\sym{***}\\
                    &                     &     (0.002)         &     (0.002)         &     (0.003)         &                     &     (0.010)         \\
Joint significance  &                     &       0.000         &       0.000         &       0.000         &                     &       0.000         \\
Vertex              &                     &       5.135         &       5.073         &       5.027         &                     &       4.881         \\
R-squared           &       0.355         &       0.192         &       0.277         &       0.456         &       0.639         &       0.726         \\
Observations        &        1086         &        1086         &        1086         &        1086         &         945         &         945         \\


==> table4C.tex <==
Position on multiculturalism&      -0.065\sym{***}&       0.474\sym{***}&       0.467\sym{***}&       0.420\sym{***}&      -0.092\sym{**} &       0.918\sym{***}\\
                    &     (0.014)         &     (0.049)         &     (0.054)         &     (0.037)         &     (0.043)         &     (0.118)         \\
Position on multiculturalism sq.&                     &      -0.048\sym{***}&      -0.048\sym{***}&      -0.043\sym{***}&                     &      -0.093\sym{***}\\
                    &                     &     (0.005)         &     (0.005)         &     (0.004)         &                     &     (0.012)         \\
Joint significance  &                     &       0.000         &       0.000         &       0.000         &                     &       0.000         \\
Vertex              &                     &       4.952         &       4.919         &       4.825         &                     &       4.943         \\
R-squared           &       0.398         &       0.194         &       0.361         &       0.506         &       0.678         &       0.756         \\
Observations        &        1087         &        1088         &        1088         &        1087         &         946         &         946         \\


==> table5.tex <==
Centrism econ       &       0.565         &      -0.324         &                     &                     \\
                    &     (0.438)         &     (1.148)         &                     &                     \\
Centrism econ $\times$ corruption&       0.004         &       0.020         &                     &                     \\
                    &     (0.006)         &     (0.017)         &                     &                     \\
Extremism social    &                     &                     &       0.846\sym{***}&       0.910\sym{*}  \\
                    &                     &                     &     (0.224)         &     (0.481)         \\
Centrism social $\times$ corruption&                     &                     &       0.002         &      -0.004         \\
                    &                     &                     &     (0.003)         &     (0.007)         \\
R-squared           &       0.443         &       0.898         &       0.656         &       0.902         \\
Observations        &         406         &         212         &         406         &         214         \\


==> table6.tex <==
Centrism on economic issues&       0.567\sym{***}&       0.661\sym{***}&                     &                     \\
                    &     (0.095)         &     (0.186)         &                     &                     \\
Centrism on econ $\times$ dissent on econ&                     &      -0.038         &                     &                     \\
                    &                     &     (0.062)         &                     &                     \\
Centrism on social values&                     &                     &       0.809\sym{***}&       0.557\sym{***}\\
                    &                     &                     &     (0.101)         &     (0.129)         \\
Centrism on social $\times$ dissent on social&                     &                     &                     &       0.112\sym{**} \\
                    &                     &                     &                     &     (0.048)         \\
Joint significance  &                     &                     &                     &                     \\
Vertex              &                     &                     &                     &                     \\
R-squared           &       0.533         &       0.534         &       0.686         &       0.695         \\
Observations        &         272         &         272         &         267         &         267         \\


==> table7.tex <==
Centrism on economic issues&       0.832\sym{***}&       0.845\sym{***}&                     &                     \\
                    &     (0.075)         &     (0.083)         &                     &                     \\
Centrism $\times$ most seats&                     &      -0.199         &                     &                     \\
                    &                     &     (0.335)         &                     &                     \\
Centrism on social values&                     &                     &       0.967\sym{***}&       0.933\sym{***}\\
                    &                     &                     &     (0.053)         &     (0.057)         \\
Centrism $\times$ most seats&                     &                     &                     &       0.322\sym{*}  \\
                    &                     &                     &                     &     (0.169)         \\
Most seats          &       0.088         &       0.692         &       0.428\sym{**} &      -0.444         \\
                    &     (0.215)         &     (1.046)         &     (0.183)         &     (0.425)         \\
R-squared           &       0.466         &       0.467         &       0.668         &       0.672         \\
Observations        &         385         &         385         &         384         &         384         \\

